Understanding Multimodal Procedural Knowledge by Sequencing Multimodal Instructional Manuals

The ability to sequence unordered events is an essential skill to comprehend and reason about real world task procedures, which often requires thorough understanding of temporal common sense and multimodal information, as these procedures are often communicated through a combination of texts and images. Such capability is essential for applications such as sequential task planning and multi-source instruction summarization. While humans are capable of reasoning about and sequencing unordered multimodal procedural instructions, whether current machine learning models have such essential capability is still an open question. In this work, we benchmark models' capability of reasoning over and sequencing unordered multimodal instructions by curating datasets from popular online instructional manuals and collecting comprehensive human annotations. We find models not only perform significantly worse than humans but also seem incapable of efficiently utilizing the multimodal information. To improve machines' performance on multimodal event sequencing, we propose sequentiality-aware pretraining techniques that exploit the sequential alignment properties of both texts and images, resulting in > 5% significant improvements.

==> figs/knn_qual.tex <==
\begin{figure*}[t!]

\begin{subtable}{\textwidth}
\centering
\centering
    \includegraphics[width=.9\columnwidth]{figs/imgs/knn_1.pdf}
\caption{\footnotesize Top Retrieved Steps Sample 1}
\label{fig:ret_1}
\end{subtable}

\begin{subtable}{\textwidth}
\centering
\centering
    \includegraphics[width=.9\columnwidth]{figs/imgs/knn_2.pdf}
\caption{\footnotesize Top Retrieved Steps Sample 2}
\label{fig:ret_2}
\end{subtable}

\vspace{.5em}

\caption{ \footnotesize
    \textbf{Exemplar manual completion task samples:}
    \textbf{(a) (b)} We show two representative zero-shot manual completion examples.
    In each successful example, where the model correctly retrieves the ground truth step and is able to properly infer its original missing position, we additionally show other top-3 retrieved candidates beside the ground truths.
    These additional candidates show interesting semantic coherence with the ground truth step, where it shows semantically coherent step description (\textcolor{blue}{highlight in blue}) and associated images.
    We truncate some of the instructions to fit the figures, and these examples are obtained from the best multimodal model, VisualBERT$\dagger$ + BERSON.
}
\label{fig:ret}
\end{figure*}

==> figs/multi_to_uni.tex <==
\begin{figure*}[t!]

\begin{subtable}{\textwidth}
\centering
\centering
    \includegraphics[width=.95\columnwidth]{figs/imgs/multi_to_uni_1.pdf}
\caption{\footnotesize Multimodal Success Sample 1}
\label{fig:multi_to_uni_1}
\end{subtable}

\begin{subtable}{\textwidth}
\centering
\centering
    \includegraphics[width=.95\columnwidth]{figs/imgs/multi_to_uni_2.pdf}
\caption{\footnotesize Multimodal Success Sample 2}
\label{fig:multi_to_uni_2}
\end{subtable}

\vspace{.5em}

\begin{subtable}{\textwidth}
\centering
\centering
    \includegraphics[width=.95\columnwidth]{figs/imgs/multi_to_uni_3.pdf}
\caption{\footnotesize Multimodal Failure Sample}
\label{fig:multi_to_uni_3}
\end{subtable}

\caption{\footnotesize
    \textbf{Exemplar qualitative model predictions:} The results above dotted blue lines are obtained from the text-only model and the below is from the multimodal model. \textbf{(a)} \textbf{(b)} demonstrates two representative cases when multimodal models outperform text-only counterparts. The textual descriptions can contain certain ambiguity such that models can wrongly infer the sequential order. For instance \textit{"cut another notch..."} is predicted to be right after \textit{"cut a notch in one side..."} by the text-only model in example (a). \textbf{(c)} We also show a failure case of multimodal models, where the image sequence may be misleading to the model. For instance, there can be many manuals where using a clipper to clip an egg precedes putting it to boil.
}
\label{fig:multi_to_uni}
\end{figure*}

==> figs/top_3_categories_uni_multi.tex <==
\begin{figure}[t!]
\centering
    \includegraphics[width=1.0\columnwidth]{figs/imgs/table2.pdf}
    \caption{
    \footnotesize
    \textbf{Top and least-3 categories of \textbf{uni-multi-modal} performance difference:} Performance are measured by PMR using the best text-only and multimodal models. The selected categories have~\textgreater10 samples in the golden-test-set. Darker colored regions indicate that multimodality have significant benefits over the unimodal (text-only) counterparts.
    }
    \label{fig:uni_multi_cats}
\end{figure}

==> old_text/abstract.tex <==
\iffalse
\all{inline comments: check macro.tex}

\telin{sample}
\alex{sample}
\marjorie{sample}
\ralph{sample}
\nanyun{sample}

\all{sidenotes: add an s to inline ones}

\telins{sample side note}
\fi
% \all{useful reference macro: figref, tbref, secref, check macro.tex}

% \telin{Check all figs are mentioned in the text, no citations and references missing (fig refs, sections refs etc.).}

% \telin{Check all the spellings, grammars, etc. For the final few passes.}

% \telin{Enlarge text in figures (charts)}

% \telin{Check all the bibtex}
\iffalse
Understanding and reasoning about sequencing steps is crucial for enabling machines to plan and accomplish complex tasks.
Given a set of (unordered) instructions, it requires understanding of event causality and temporal common sense reasoning to infer the proper order of subtasks.  Instructions for complex tasks are often multimodal, where textual descriptions are supplemented by images for more detailed guidance.
In this work, we scrape a widely-used instructional manual, WikiHow, and convert an existing data resource, RecipeQA, for benchmarking the capabilities of NLP and multimodal models on the multimodal procedure sequencing task.
Additionally, we establish human evaluation for the two datasets.
Our studies on both the model and human performance and their analysis shows that multimodality is indeed helpful for sequencing procedures and suggests potential future directions to bridge the gap between model and human performance.
\fi
% on the multimodal procedure understanding task.

% NOTE THE FOLLOWING IS EDIT FROM MARJORIE
% \telins{inline comments: check macro.tex}
Human knowledge about how to perform a task (\eg ``how to make a wood sign'') is often communicated through a set of procedural instructions in a combination of text and images.
Reasoning about the sequentiality of task procedures can facilitate sequential task planning and multi-source instruction summarization.
% how to accomplish the task requires understanding event temporal and causal relations.
In this work, we investigate the degree to which machines are able to reason about task-order when presented with text or multimodal data. We curate two multimodal datasets that contain rich procedural information. %where the steps in an instruction are presented in a scrambled form to the machine that is asked to assign the proper order.
The datasets are drawn from online instructional manuals, including WikiHow and Recipes.
We benchmark language only and multimodal models' ability to understand procedural processes by presenting them with a scrambled form of the procedural sequences and asking them to restore the proper order. We measure models' accuracies on this sequencing task and establish human performance for the two datasets.
Our studies show that multimodal information is helpful for sequencing procedures, and procedural knowledge understanding helps the downstream application of manual completion.
% \violet{missing step retrieval(?)}.
% Further analysis shows that \violet{add some insights/take home message here.}
%Additionally, we conduct model analysis and demonstrate a downstream application of sequencing task-orders.
% \nanyuns{the last sentence is too long... maybe break it into two?}

==> old_text/ethics.tex <==
\section{Ethics and Broader Impacts}

We hereby acknowledge that all of the co-authors of this work are aware of the provided \textit{ACM Code of Ethics} and honor the code of conduct.
This work is mainly about sequencing a given series of multimodal task procedures, represented by text descriptions along with their images.
The followings give the aspects of both our ethical considerations and our potential impacts to the community.

\vspace{.3em}

\mypar{Dataset.} We collect the human performance on our sequencing task via Amazon Mechanical Turk (MTurk) and ensure that all the personal information of the workers involved (e.g., usernames, emails, urls, demographic information, etc.) is discarded in our dataset.
This research has been reviewed by the \textbf{IRB board} and granted the status of an \textbf{IRB exempt}.
The detailed annotation process (pay per amount of work, guidelines) is included in the appendix; and overall, we ensure our pay per task is above the the annotator's local minimum wage (approximately \$12 USD / Hour).
We primarily consider English speaking regions for our annotations as the task requires certain level of English proficiency.

\vspace{.3em}

\mypar{Techniques.} We benchmark the sequencing tasks with the state-of-the-art large-scale pretrained language and multimodal models.
As commonsense and task procedure understanding are of our main focus, we do not anticipate production of harmful outputs, especially towards vulnerable populations, after training models on our proposed task.

==> old_text/experiments.tex <==
\section{Experiments and Analysis}

\vspace{-.5em}

% \telin{Opening paragraph with some research questions: (1) How valid the task is, e.g. human performance, (2) how much can models do, (3) certain analysis.}
Our experiments seek to answer the following research questions:
(1) How valid is the proposed task for humans to complete?
(2) Is multimodality helpful? When?
(3) Can sequencing benefit downstream tasks that require procedural knowledge?
% \violet{(3) Can procedure understanding benefit downstream tasks?}

\vspace{-.5em}

\subsection{Evaluation Metrics}
% \telin{Describe our evaluation metrics used in this work.}
\vspace{-.3em}

We adopt metrics below following existing works:
\iffalse
\begin{itemize}[leftmargin=*]
    \item \textbf{Matching-based:} (1) partial match (PM) ... (2) exact match (EM)
    \item \textbf{LCS:} ...
    \item \textbf{Minimum-Swapping:} (Kendal's $\tau$)...
\end{itemize}
\fi

% \input{tables/dataset_stats}
\input{tables/model_performances}

\mypar{Position-Based} We consider:
1) Accuracy (Acc) which computes the ratio of absolute positions in the ground truth procedure order that are correctly predicted;
2) Perfect Match Ratio (PMR) which measures the percentage of predicted orders exactly matching the ground truths;
and 3) Distance (Dist) which measures average distance\footnote{Except for distance metric, higher scores are better.} between the predicted positions of each step to its ground truth position.
% for indicating model performance on predicted positions of a sequence.

\mypar{Longest Common Subsequence:} which computes the ratio of longest common subse\textbf{q}uence~\cite{gong2016end} between the predicted and ground truth procedure orders (L$_{q}$). We also consider a stricter version which requires the consecutiveness for the comparisons, longest common subst\textbf{r}ing (L$_{r}$).

\mypar{Kendall's Tau ($\tau$):} which is defined as
$1 - 2\times (\#\ inversions) / (\#\ pairs)$, where the inversion means that the relative predicted order of a pair is incorrect (inverted to the ground truth pair) and $\#\ pairs = {N \choose 2}$ ~\cite{lapata2003probabilistic}.

\vspace{-.3em}
\subsection{Human Annotations}
\vspace{-.3em}

% \telin{Describe the detailed procedures of obtaining the human performance, and their essential statistics and/or analysis.}
%To validate the proposed sequencing task constructed by the two targeted datasets, as well as study how multimodality is utilized, w
We perform human evaluations via Amazon Mechanical Turk.
Since our benchmark dataset is constructed from datasets that are not designed for our sequencing task, the quality of random samples is unverified.
To construct a high quality human-annotated test set, we manually select 300 samples in WikiHow and 100 samples in RecipeQA, using the aforementioned criteria: procedural in both texts and images and complementary multimodal information.
%
% In addition to labelling the correct order of the scrambled manual,
Apart from the sequencing task, we also ask the annotators for their confidence of predictions and if multimodality is helpful for deciding the order.
For more details, see ~\appendixref{a-sec:human}.

\vspace{-.3em}
\subsection{Experimental Setups}
\vspace{-.3em}

% \telin{Data splits, sequence length, and other essential details.}
Each step description has maximally $5$ sentences, as in the human evaluations; the maximum length per step is $60$ wordpieces. %In this work we only consider maximally $5$ steps.
For RecipeQA we use the original data splits.
To prevent models' exploiting category-level knowledge, WikiHow is split so that certain categories do not overlap in each split.

% \violet{can probably move this entire paragraph to the appendix for space.}
% \mypar{Train-Test Splits:} For RecipeQA we use the original data splits which ensure no identical recipe appears in more than one set. For WikiHow, we split the data according to the third level category\footnote{Prevent models from exploiting too similar task knowledge in the same category, the level is empirically decided.}, \ie no articles belonging to the same third-level category should appear in more than one set. We also prioritize categories that are more likely to be procedural (concerning more physical knowledge) for the test sets (See~\secref{a-sec:dataset_stats} for more details).

\vspace{-.3em}
\subsection{Results and Analysis}
\vspace{-.3em}

\tbref{tab:model_performances} summarizes the model performance on the human annotated test set\footnote{We include results for other splits in~\appendixref{a-sec:dev_set}.}.
In both datasets, the two multimodal models consistently outperform their text-only counterparts. 
The domain-adapted pretraining is effective for all the benchmark models.
The BERSON ordering module performs significantly better than pairwise learning model, followed by topological sort. This signifies the importance of global as well as local context. 

However, we observe a gap between our top-performing model and human performance, especially in the PMR metric. Additionally, we observe a significantly larger gap in human performance between text-only vs. multimodal than we do in model performance. We hypothesize that grounding languages to perform finer-grained~\textit{visual co-reference} can facilitate multimodal sequential understanding, which is left as a future work.
% (2) The gap between the Acc and PMR metric, as well as the L$_{seq}$ and L$_{str}$ metrics are smaller that those of the models, indicating more robust judgements from the humans.

% \subsection{Analysis}

\vspace{.3em}

\mypar{Category Analysis.}
In~\figref{fig:cats} we select the top three WikiHow categories in which multimodal models outperform the text-only counterparts the most, and vice versa, using the PMR metric.
% (\ie more social and personal).
The observation aligns with our intuitions that models benefit from multimodality on tasks that follow a definite order (\ie procedural data, like a physical category), compared with tasks that do not, where visual information may, on the contrary, be misleading. For examples, see~\appendixref{a-sec:quali}.

% \input{tables/categories}
\vspace{.3em}

\mypar{Zero-Shot Manual Completion.}
One potential downstream application for task-order sequencing is to infer the missing steps in an \textit{incomplete} instructional manual.
For each task in the human test set, we randomly \textit{skip a step} and provide the rest of the steps to a trained model in \textit{ground truth order}.
The model is then asked to retrieve the missing step from a step pool composed by all the steps in this dataset.
Using a trained model, we take the `[CLS]' output representations of both the incomplete manual and each step in the pool to perform a \textit{zero-shot} nearest neighbor search\footnote{We feed the incomplete manual at once to the retrieval model and mean pool the step-wise {\tt `[CLS]'} representations.}.
We compute the mean reciprocal rank (MRR) and Top-1 accuracy for such step retrieval.
Additionally, we evaluate whether the model can \textit{identify} which step is missing by correctly ``putting" the retrieved step back to \textit{complete} a proper manual, via the learned sequencing capability\footnote{Sequencing is performed with appending the retrieved step to the end of the incomplete manual.}.
We compute a \textit{mean reciprocal step recognition} (MRSR) as:
$\frac{\mathds{1}[\text{correct prediction}]}{\text{rank of gt}}$.
The results shown in~\tbref{tab:zero_shot} suggests that multimodality is likewise helpful in this downstream task.

\input{figs/top_3_categories}
\input{tables/zero_shot_ret}

% \telin{To be added.}

% \telin{Maybe some interesting retrieval-based examples. To show that the retrieved items are meaningful, which can drive the future works for task graphs.}

% \noindent \telin{More ideas?}

==> old_text/intro.tex <==
\section{Introduction}
% \telins{Make sure the terminologies are consistent throughout the whole paper, eg. pretrained, hyper-parameters, finetuned, ... etc.}

\iffalse
\telin{
Flow:

(1) An opening paragraph to motivate procedural understanding is important in NLP research and/or multimodal research. Refer to the teaser figure with a good example to draw the connection between the sequencing task to common sense, temporal understanding and procedure construction. Define the problem of the multimodal sequencing task.

(2) Mention prior works mostly focus on sentence ordering (and maybe less instructive type? More like stories or paper abstract), and one closely related work SortStory concerns multimodal inputs. But SortStory utilizes VIST dataset which is not very desiring (explain) as we look for better dataset that features: 1) events are procedural in both texts and visuals, and 2) multimodal inputs complement each other more.

(3) And hence we put forth to transform some existing dataset (RecipeQA) and scrape popular instructional dataset (WikiHow) to create the testbed for our proposed sequencing task. Explain in more details about the data and their traits/features. And explain our human annotations for the validity of the task.

(4) Models. The models we evaluate on this testbed is of base model-and-ordering module style. For the base models we leverage language models and two multimodal models, and for the ordering module we leverage conventional sorting and BERSON.

(5) A paragraph about experiments and brief performance mentioning. And then conclude this paragraph with a summary our contributions:
1) Create a better testbed to evaluate multimodal procedure understanding,
2) Human performance analysis,
3) Model benchmarking and future work motivations.
}
\fi

Humans often refer to instructions to complete a complex tasks composed of multiple steps, such as \textit{making a wood sign from scratch}.
However, instructions can be obtained from multiple different sources, and hence do not always come in a proper sequential order.
%Furthermore, in situations such as multitasking, humans have developed the ability to reason about task sequences that are not in proper sequential order \cite{bode2009decoding, broeker2018multitasking}.
Thus, sequencing \textit{unordered} tasks is crucial for comprehending and inferring task procedures, where it requires thorough understanding of event causal and temporal common sense. Progress in task sequencing can help filling incomplete task instructions and robot task planning~\cite{garattoni2018autonomous}.

Existing work has studied task sequencing by sorting sentences from paper abstracts or short stories~\cite{chen2016neural, cui2018deep, logeswaran2018sentence, oh2019topic, lee2020slm}. However, real-life tasks are often complex: multimodal information often provides additional cues when textual descriptions exhibit ambiguity or omit implicit details, as illustrated in~\figref{fig:teaser}.% Sequencing such tasks is still under explored.
% and script generation~\cite{wang2017integrating}.
% In computer vision, sequencing video frames is shown to learn useful representations~\cite{lee2017unsupervised, li2020hero}.

Prior work also attempts to extend the sequencing task to multimodal data~\cite{agrawal2016sort}.
However, the dataset used, Visual StoryTelling~\cite{huang2016visual}, merely targets \textit{short human created stories}; the featured images were not intended to be procedural (or temporally coherent) nor supply unstated details to the texts\footnote{The images come from photo albums and the annotators \textit{create} stories based on their freely arranged image sequences.}.
% However, the images in the employed dataset, Visual StoryTelling~\cite{huang2016visual}, were either not intended to be procedural (and temporally coherent) or created to supply unstated details to the texts\footnote{The images come from photo albums and the annotators \textit{create} stories based on their freely arranged image sequences.}.

\input{figs/teaser}

To investigate how current AI techniques can understand procedural knowledge and leverage multimodality to facilitate reasoning, we consider the sequencing task with \textit{online instructional manuals}.
We curate two representative instruction resources, a ``How-To" instructions (WikiHow) and cooking recipes; we establish human evaluations on a selected subset for each data resource.
We construct models which consist of:
(1) a base model to encode either text-only or multimodal inputs, 
and (2) an ordering module which predicts proper step order from the output of the base model,
for the benchmark purpose.
%
We employ RoBERTa~\cite{liu2019roberta} and two popular multimodal models, ViL-BERT~\cite{lu2019vilbert} and VisualBERT~\cite{li2019visualbert} as base models.
To predict the step order, we integrate the base models into recent sentence ordering frameworks: pairwise constraint learning with topological sort~\cite{prabhumoye2020topological} and BERSON~\cite{cuietal2020bert}.

% \violet{I'll merge this into the contribution list. Here I'll start with summarizing the contribution: 1) investigating model and human performance on sequencing multimodal inputs, experiments show that xxx, give some insights/take home message. 2) We provide analysis. 3) downstream application (although one issue is that this step 3 is disconnected from the first two -- it's unclear to me why would we do 3) after we see the results from 1) and 2)...)}

Our key contributions are:
(1) we investigate the model performance on sequencing scrambled manuals, where we show multimodality increases performance
%is helpful on such procedure understanding task
yet we find a significant gap (\textgreater15\%) below human performance,
(2) we provide analysis on when multimodality is most helpful,
and (3) we demonstrate a downstream application where procedure knowledge learned from the sequencing task is beneficial.

\iffalse
Our experiments show that, compared to human performance, models struggle in sequencing with a gap of~\textgreater15\% in perfect match ratio.
\violet{would be good if we can draw some insights about why this gap exists.}
We provide analysis on when multimodality is most helpful, and devise a downstream application to complete task manual.
In summary, our contributions are:
(1) investigating model and human performance on sequencing multimodal inputs,
(2) analysis and insights on multimodality,
and (3) downstream applications and motivating future research.
\fi

==> old_text/models.tex <==
\section{Models}
% \telin{A general paragraph for the models, including (1) Multimodality, (2) Encoder-Decoder style, where the decoder decodes the actual order.}

The model, which takes as inputs a set of \textit{scrambled} task-steps and predicts the appropriate order,
% considered for the proposed multimodal sequencing task
consists of two major components:
(1) a \textbf{base model} which encodes the textual and/or multimodal inputs,
and (2) an \textbf{ordering module} which operates on top of the base model to produce the order.

\subsection{Base Models}

\mypar{Text-Only Models.}
We use RoBERTa~\cite{liu2019roberta}, an optimized variant of BERT language model~\cite{devlin2019bert}, for text-only inputs.

\vspace{.3em}

\mypar{Multimodal Models.}
We consider the following two visual-linguistics BERT-style models because they are easily adaptable to our sequencing task\footnote{\citet{bugliarello-etal-2020-multimodal} suggests that many V\&L models can achieve similar downstream performance if well trained.}:
% Note that we specifically choose one model from two-stream and the other from the single-stream model families, differed by whether they fuse the multimodal inputs in an late or early fusion manner.
% \telins{change according to Wade's suggestions}
\vspace{-.3em}
\begin{itemize}[leftmargin=*]
    \item \textbf{ViL-BERT}~\cite{lu2019vilbert} learns a joint visual-and-linguistics representation through co-attentional transformer layers. ViL-BERT is pretrained with: (1) multimodal masked learning (MLM), and (2) image-text alignment prediction (ITM). In ITM, images are randomly replaced with others to create misalignment, which the model trains on.
    % \vspace{-1.9em}
    \item \textbf{VisualBERT}~\cite{li2019visualbert} grounds the image regions to language with a single transformer model~\cite{vaswani2017attention}. It is also pretrained with multimodal MLM and ITM. %sentence-image-matching prediction objectives (ITM).
\end{itemize}

\subsection{Ordering Modules}

\mypar{Topological Sort.}
% A straightforward ordering algorithm is to 
As a baseline, we first construct a directed graph between steps where the direction indicates the relative order of the steps (\ie $s_i \rightarrow s_j$ indicates step $s_i$ precedes $s_j$), and then apply topological sort~\cite{tarjan1976edge}. Similar to~\cite{prabhumoye2020topological}, we train the base models to perform a binary relative order prediction (\ie whether $s_i \rightarrow s_j$ or $s_i \leftarrow s_j$) by feeding a pair of (text and multimodal) inputs, separated by the '[SEP]' special token.
If a cycle (which should not result from in an ideal pairwise prediction model) is detected by the depth-first-search-based topological sort algorithm, we break the cycle at the pair with lowest predicted softmax probability, \ie $\argmin_i P(s_{c_i} \rightarrow s_{c_{i+1}})$ where ${c_i}$ is the index of the elements in that cycle.

\vspace{.3em}

\mypar{BERSON}
is a recently proposed state-of-the-art neural sentence ordering framework~\cite{cuietal2020bert}, where a pointer network~\cite{vinyals2015order} exploits both the local (relative pairwise order) and global (self-attentions on top of the entire input sequence) information of the inputs to decode the predicted order.
As BERSON utilizes the next sentence prediction objective in the BERT model, we use the aforementioned pairwise-trained base models to integrate with BERSON.

% \subsubsection{Approximated Sorting}

\subsection{Implementation and Training Details}

\mypar{Domain Adapting Pretraining:}~\cite{dontstoppretraining2020}
% \telin{General procedure: (1) Pretraining on the datasets with multimodal models undergo ViL-BERT-style pretraining. (2) Finetuning with sequence labels. (3) Inference.}
We also attempt to pretrain the base models on the two datasets to adapt them from their pretrained domains to the targeted dataset domains.
Additionally, to train the models to understand sequences of images, we adopt the following modifications:
% facilitate the sequentiality understanding of the images, the pretraining of the two multimodal models adopts the following modifications:
(1) We concatenate all the step descriptions (each with its own {\tt `[CLS]'} and {\tt `[SEP]'} tokens) with the whole image sequence at once, following the original order. % , to form a joint description text.
(2) The ITM is modified by
% replacing the text (or image) with a randomly sampled one, this would be analogous to
replacing the whole image sequence from another manual in the dataset. % Instead, our ITM is performed by only \textit{replacing a subset of the image sequence}, which requires better multimodal sequentiality understanding from the models.
This pretraining is only conducted on the training set.

\mypar{Image Features:}
Due to memory and computational concerns, for each image we include the whole image features and top-$3$ ROI pooled image regional features\footnote{Ranked by the objectness and recognition scores.} from an object detection module.

\iffalse
\mypar{Pretrained Weights:}
% \telin{Potential details of the parameters initialization, model checkpointing, and referring to appendix for more details.}
All the base models are initialized with their respective large-scale pretrained weights, and we use Faster-RCNN with feature pyramid networks~\cite{lin2017feature} for encoding the images.
More details are in~\secref{a-sec:impl}.
\fi

==> old_text/related_works.tex <==
\section{Related Works}

\mypar{Neural Ordering.}

\vspace{0.3em}

\mypar{Procedure Understanding.}

\vspace{0.3em}

\mypar{Multimodality.}


==> old_text/task.tex <==
\section{Datasets}

\iffalse
\mypar{Problem Definition.} 
% \telin{Define the problem and terminologies/notations throughout the paper.}
Given a task procedure $S$ consisting of $N$ steps, where each step $s_i \in S$ is multimodally represented by a textual description and corresponding image(s), a model is required to take as inputs a random permutation of $S$ (\ie $S_p = \{s_{p_1}, ..., s_{p_N}\}$, where $p$ is a permutation) and predict the correct integer order of $S_p$.
\fi

% \subsection{Datasets}

% \telin{A paragraph to describe that the data we are looking for needs to be: (1) Procedural in both texts and visuals. (2) Texts and visuals are intended to complement each other. (3) The aspects in common sense that we care about: physical, social.}

There are three major features we require from the target dataset:
(1) It is multimodal.
(2) It consists of task procedures as sequences of steps, where each modality shows clear \textit{procedural characteristics}.
% \telins{Counter the VIST in SortStory more?}
(3) Different modalities are used intentionally to complement each other.
In light of these, we consider the two following datasets:

\vspace{.3em}

\mypar{RecipeQA}
% \telin{Details of the RecipeQA dataset and our transformation.}
% \telin{Quick statistics?}
is a multimodal question answering dataset consists of numerous recipes scraped from \textit{Instructables.com} \cite{yagcioglu2018recipeqa}.
We utilize the recipes collected in this dataset as they are inherently procedural and multimodal.

% We utilize RecipeQA by converting each unique recipe into sequential multimodal steps for our sequencing task.

\vspace{.3em}

\mypar{WikiHow}
% \telin{Details of the WikiHow dataset.}
% \telin{The scraping and cleaning procedures.}
% \telin{The hierarchy information.}
% \telin{The difference between ours and the abstractive WikiHow dataset as a contribution?}
% \telin{Quick statistics?}
is an online knowledge base that consists of human-created articles describing procedures to accomplish a desired task.
Each article contains a high level goal of a task (\eg ``How To ..."), a short summary of the procedures introduced, and several \textit{multimodal} steps where each step consists of a description paired with one or a few corresponding images and/or gifs.
Prior works have utilized WikiHow for several NLP tasks, including
abstractive summarization~\cite{koupaee2018wikihow}, and task knowledge learning~\cite{zhou-etal-2019-learning-household,tandon-etal-2020-dataset, zhang-etal-2020-intent}.
\citet{zhang-etal-2020-reasoning} also considers WikiHow for learning event temporal ordering, but with a limitation of only handling pairwise relative order.

As WikiHow includes multimodal information for task knowledge, concurrent work also uses it as a resource for understanding visual goals~\cite{yang2021visual}.
However, we are the first to consider WikiHow as a resource for a comprehensive multimodal procedural understanding.
We scrape the entire WikiHow knowledge base, containing more than 100k unique articles along with most of its multimodal contents\footnote{The dataset and relevant tools will be made public.}, as well as the hierarchical category (\ie subcategory paths) for each article.
For details, see~\appendixref{a-sec:dataset_stats}.

==> tables/alternative_order_modality_quad.tex <==
\begin{table}[t!]
\centering
\footnotesize
% \scalebox{.88}{
    \begin{tabular}{cc|cc}
    \toprule
    \multicolumn{2}{c}{\multirow{2}{*}{\textbf{Modality}}}  & \multicolumn{2}{c}{\multirow{1}{*}{\textbf{Multimodal}}} \\
                                                            &   & Y   & N   \\
    \midrule % \\[-1.1em]
    \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Text-Only}}} & Y & 29  & 20 \\
                                                            & N & 22  & 229 \\
    \bottomrule
    \end{tabular}
% }
\caption{
\footnotesize
\textbf{Modality Quad Table:} ...
}
\label{tab:alternative_modality_quad}
\end{table}

==> tables/categories.tex <==
\begin{table}[t!]
\centering
\small
\scalebox{.9}{
    \begin{tabular}{l|ccc}
    \toprule
    Categories & PMR$_{\text{multi}}$ & PMR$_{\text{text}}$ & Diff. \\
    \midrule % \\[-1.1em]
    
    % Human Test Set.
    \multirow{1}{*}{Computers and Electronics}
    & 45.45 & 31.82 & 11.63 \\
    \multirow{1}{*}{Home and Garden}
    & 63.86 & 55.42 & 8.44 \\
    \multirow{1}{*}{Hobbies and Crafts}
    & 46.51 & 39.53 & 6.98 \\
    \cline{1-4}\\[-.8em]
    \multirow{1}{*}{Personal Care and Style}
    & 29.41 & 41.18 & -11.77 \\
    \multirow{1}{*}{Arts and Entertainment}
    & 46.15 & 53.85 & -7.70 \\
    \multirow{1}{*}{Health}
    & 31.25 & 37.50 & -6.25 \\

    \bottomrule
    \end{tabular}
}
\caption{
\footnotesize
\textbf{Top-3 Categories of performance difference:} The selected categories have~\textgreater10 samples in the human test set. The subscripts multi and text indicates the performance obtained from either the multimodal model (VisualBERT$\dagger$ + BERSON) or text-only model (RoBERTa$\dagger$ + BERSON). 
}
\label{tab:cats}
\end{table}

==> tables/dataset_stats.tex <==
\begin{table}[t!]
\centering
\small
% \scalebox{.88}{
    \begin{tabular}{c|cccc}
    \toprule
    \textbf{Dataset} & Train & Dev & Test & Human \\
    \midrule % \\[-1.1em]
    RecipeQA & 8032 &  973  & 1058 & 100 \\
    WikiHow  & 98268 & 5459 & 5759 & 300 \\
    \bottomrule
    \end{tabular}
% }
\caption{
\footnotesize
\textbf{Dataset Statistics:} Number of unique manuals (recipes) in each dataset split. Note that the human test set is a subset of the test set itself.
}
\label{tab:dataset_stats}
\end{table}

==> tables/model_performances_dev.tex <==
\begin{table*}[t!]
\centering
\small
\scalebox{.845}{
    \begin{tabular}{cc|cccccc|cccccc}
    \toprule
    \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Modality}}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Models}}} & \multicolumn{6}{c}{\textbf{WikiHow Dev \& Test Set}} & \multicolumn{6}{c}{\textbf{RecipeQA Dev \& Test Set}} \\
    % & & & PM$\uparrow$ & EM$\uparrow$ & $\tau\uparrow$ & LC$_{\text{seq}}\uparrow$ & LC$_{\text{str}}\uparrow$ & Dist.$\downarrow$ & PM$\uparrow$ & EM$\uparrow$ & $\tau\uparrow$ & LC$_{\text{seq}}\uparrow$ & LC$_{\text{str}}\uparrow$ & Dist.$\downarrow$ \\
    & & Acc$\uparrow$ & PMR$\uparrow$  & L$_{q}\uparrow$ & L$_{r}\uparrow$ & $\tau\uparrow$ & Dist$\downarrow$ & Acc$\uparrow$ & PMR$\uparrow$ & L$_{q}\uparrow$ & L$_{r}\uparrow$ & $\tau\uparrow$ & Dist$\downarrow$ \\
    % & & \textbf{Acc} & \textbf{PMR}  & \textbf{L$_{seq}$} & \textbf{L$_{str}$} & \textbf{$\tau$} & \textbf{Dist.} & \textbf{Acc} & \textbf{PMR}  & \textbf{L$_{seq}$} & \textbf{L$_{str}$} & \textbf{$\tau$} & \textbf{Dist.} \\
    \midrule % \\[-1.1em]
    
    \multirow{1}{*}{Image-Only}
    & \multirow{1}{*}{FRCNN + BERSON}
      & 21.84 & 1.20 & 2.87 & 1.77 & 0.04 & 7.73 & 32.64 & 4.40 & 3.23 & 1.94 & 0.26 & 6.06 \\
    \midrule
    
    \multirow{5}{*}{Text-Only}
    & \multirow{1}{*}{RoBERTa + TopoSort}
      & 48.61 & 20.50 & 3.77 & 2.59 & 0.55 & 3.98 & 55.71 & 25.98 & 3.97 & 2.81 & 0.65 & 3.18 \\
    & \multirow{1}{*}{RoBERTa$\dagger$ + TopoSort}
      & 46.73 & 19.39 & 3.71 & 2.55 & 0.51 & 4.26 & 61.30 & 34.44 & 4.10 & 3.06 & 0.70 & 2.73 \\
    \cline{2-14} \\[-.8em]

    & \multirow{1}{*}{BERT + BERSON}
      & 53.40 & 28.88 & 3.93 & 2.94 & 0.57 & 3.75 & 61.24 & 35.20 & 4.09 & 3.11 & 0.68 & 2.84 \\
    & \multirow{1}{*}{RoBERTa + BERSON}
      & 54.97 & 28.28 & 3.94 & 2.87 & 0.60 & 3.47 & 63.41 & 38.07 & 4.17 & 3.22 & 0.72 & 2.57 \\
    & \multirow{1}{*}{RoBERTa$\dagger$ + BERSON}
      & 59.15 & 36.11 & 4.06 & 3.13 & 0.64 & 3.15 & 65.50 & 41.09 & 4.21 & 3.29 & 0.73 & 2.43 \\
    
    \midrule

    \multirow{8}{*}{Multimodal}
    & \multirow{1}{*}{ViL-BERT + TopoSort}
      & 45.91 & 17.37 & 3.65 & 2.43 & 0.50 & 4.31 & 55.02 & 24.62 & 3.93 & 2.71 & 0.65 & 3.20 \\
    & \multirow{1}{*}{ViL-BERT$\dagger$ + TopoSort}
      & 51.40 & 24.23 & 3.83 & 2.68 & 0.58 & 3.75 & 58.67 & 29.76 & 4.00 & 2.92 & 0.67 & 2.94 \\
    & \multirow{1}{*}{VisualBERT + TopoSort}
      & 52.29 & 25.38 & 3.86 & 2.74 & 0.59 & 3.67 & 62.02 & 35.20 & 4.14 & 3.10 & 0.71 & 2.65 \\
    & \multirow{1}{*}{VisualBERT$\dagger$ + TopoSort}
      & 53.32 & 26.53 & 3.89 & 2.80 & 0.60 & 3.58 & 61.48 & 33.84 & 4.08 & 3.03 & 0.70 & 2.74 \\
    \cline{2-14} \\[-.8em]
    & \multirow{1}{*}{ViL-BERT + BERSON}
      & 56.16 & 31.97 & 3.97 & 3.01 & 0.60 & 3.51 & 61.93 & 33.69 & 4.11 & 3.08 & 0.70 & 2.69 \\
    & \multirow{1}{*}{ViL-BERT$\dagger$ + BERSON}
      & 61.13 & 38.78 & 4.10 & 3.22 & 0.66 & 3.01 & 65.56 & 41.54 & 4.24 & 3.35 & 0.73 & 2.47 \\
    & \multirow{1}{*}{VisualBERT + BERSON}
      & 59.71 & 35.38 & 4.07 & 3.12 & 0.65 & 3.09 & \textbf{67.92} & \textbf{45.17} & \textbf{4.26} & \textbf{3.44} & \textbf{0.74} & \textbf{2.32} \\
    & \multirow{1}{*}{VisualBERT$\dagger$ + BERSON}
      & \textbf{61.89} & \textbf{39.61} & \textbf{4.11} & \textbf{3.23} & \textbf{0.66} & \textbf{2.95} & 65.62 & 40.94 & 4.23 & 3.32 & \textbf{0.74} & 2.42 \\
      
    \bottomrule
    \toprule
      
    % Test Set.
    
    \multirow{1}{*}{Image-Only}
    & \multirow{1}{*}{FRCNN + BERSON}
      & 23.04 & 1.64 & 2.91 & 1.84 & 0.05 & 7.60 & 31.99 & 6.19 & 3.20 & 1.94 & 0.25 & 6.11 \\
    \midrule
    
    \multirow{5}{*}{Text-Only}
    & \multirow{1}{*}{RoBERTa + TopoSort}
      & 50.70 & 22.80 & 3.82 & 2.65 & 0.57 & 3.78 & 59.00 & 28.10 & 4.02 & 2.87 & 0.67 & 2.01 \\
    & \multirow{1}{*}{RoBERTa$\dagger$ + TopoSort}
      & 49.30 & 21.40 & 3.79 & 2.61 & 0.55 & 3.94 & 62.80 & 34.10 & 4.14 & 3.07 & 0.72 & 2.56 \\
    \cline{2-14} \\[-.8em]

    & \multirow{1}{*}{BERT + BERSON}
      & 55.90 & 31.90 & 3.98 & 3.03 & 0.60 & 3.51 & 61.20 & 33.20 & 4.10 & 3.04 & 0.68 & 2.82 \\
    & \multirow{1}{*}{RoBERTa + BERSON}
      & 57.40 & 31.20 & 4.01 & 2.98 & 0.64 & 3.21 & 65.80 & 38.86 & 4.20 & 3.24 & 0.74 & 2.37 \\
    & \multirow{1}{*}{RoBERTa$\dagger$ + BERSON}
      & 61.80 & 38.90 & 4.12 & 3.22 & 0.67 & 2.91 & 67.77 & 42.75 & 4.26 & 3.35 & 0.75 & 2.27 \\
    
    \midrule

    \multirow{8}{*}{Multimodal}
    & \multirow{1}{*}{ViL-BERT + TopoSort}
      & 47.29 & 17.04 & 3.69 & 2.43 & 0.53 & 4.08 & 54.50 & 22.70 & 3.90 & 2.63 & 0.64 & 3.21 \\
    & \multirow{1}{*}{ViL-BERT$\dagger$ + TopoSort}
      & 52.90 & 25.30 & 3.88 & 2.73 & 0.60 & 3.57 & 60.30 & 29.50 & 4.04 & 2.88 & 0.69 & 2.81 \\
    & \multirow{1}{*}{VisualBERT + TopoSort}
      & 54.70 & 26.90 & 3.93 & 2.81 & 0.62 & 3.40 & 61.60 & 32.10 & 4.09 & 2.98 & 0.70 & 2.68 \\
    & \multirow{1}{*}{VisualBERT$\dagger$ + TopoSort}
      & 55.20 & 27.80 & 3.94 & 2.84 & 0.62 & 3.38 & 62.50 & 34.60 & 4.14 & 3.11 & 0.70 & 2.69 \\
    \cline{2-14} \\[-.8em]
    & \multirow{1}{*}{ViL-BERT + BERSON}
      & 58.80 & 35.10 & 4.03 & 3.10 & 0.63 & 3.25 & 62.60 & 34.10 & 4.13 & 3.09 & 0.70 & 2.66 \\
    & \multirow{1}{*}{ViL-BERT$\dagger$ + BERSON}
      & 62.70 & 40.10 & 4.16 & 3.28 & 0.68 & 2.83 & 67.33 & 42.62 & 4.28 & 3.41 & 0.75 & 2.28 \\
    & \multirow{1}{*}{VisualBERT + BERSON}
      & 62.00 & 38.50 & 4.12 & 3.23 & 0.67 & 2.89 & 68.42 & 44.43 & \textbf{4.30} & 3.43 & \textbf{0.76} & \textbf{2.18} \\
    & \multirow{1}{*}{VisualBERT$\dagger$ + BERSON}
      & \textbf{63.70} & \textbf{41.00} & \textbf{4.15} & \textbf{3.29} & \textbf{0.69} & \textbf{2.77} & \textbf{68.96} & \textbf{45.34} & \textbf{4.30} & \textbf{3.46} & \textbf{0.76} & 2.19 \\
    
    \bottomrule
    
    \end{tabular}
}
\caption{
\footnotesize
\textbf{Development (upper half) and larger test set (lower half) performance:} The performance of the development set are mainly used to select the potentially optimal checkpoints for each model, and then evaluated on the test set and the human test set. The results on both sets also show similar trends as in~\tbref{tab:model_performances} that the multimodal models generally outperform the text-only counterparts, and the domain adapting pretraining is likewise shown to be effective.
}
\label{tab:model_performances_dev}
\end{table*}

==> tables/model_performances_old.tex <==
\begin{table*}[th!]
\centering
\small
\scalebox{.845}{
    \begin{tabular}{cr|cccccc|cccccc}
    \toprule
    \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Modality}}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Models}}} & \multicolumn{6}{c}{\textbf{WikiHow Human Test Set}} & \multicolumn{6}{c}{\textbf{RecipeQA Human Test Set}} \\
    % & & & PM$\uparrow$ & EM$\uparrow$ & $\tau\uparrow$ & LC$_{\text{seq}}\uparrow$ & LC$_{\text{str}}\uparrow$ & Dist.$\downarrow$ & PM$\uparrow$ & EM$\uparrow$ & $\tau\uparrow$ & LC$_{\text{seq}}\uparrow$ & LC$_{\text{str}}\uparrow$ & Dist.$\downarrow$ \\
    & & Acc$\uparrow$ & PMR$\uparrow$  & L$_{q}\uparrow$ & L$_{r}\uparrow$ & $\tau\uparrow$ & Dist$\downarrow$ & Acc$\uparrow$ & PMR$\uparrow$ & L$_{q}\uparrow$ & L$_{r}\uparrow$ & $\tau\uparrow$ & Dist$\downarrow$ \\
    % & & \textbf{Acc} & \textbf{PMR}  & \textbf{L$_{seq}$} & \textbf{L$_{str}$} & \textbf{$\tau$} & \textbf{Dist.} & \textbf{Acc} & \textbf{PMR}  & \textbf{L$_{seq}$} & \textbf{L$_{str}$} & \textbf{$\tau$} & \textbf{Dist.} \\
    \midrule % \\[-1.1em]
    
    % Human Test Set.
    
    \multirow{5}{*}{Text-Only}
    & \multirow{1}{*}{RoBERTa + TopoSort}
      & 60.00 & 30.70 & 4.09 & 2.98 & 0.71 & 2.78 & 69.00 & 41.00 & 4.31 & 3.37 & 0.79 & 2.02 \\
    & \multirow{1}{*}{RoBERTa$\dagger$ + TopoSort}
      & 61.40 & 32.30 & 4.11 & 3.04 & 0.71 & 2.65 & 70.00 & 42.00 & 4.28 & 3.34 & 0.79 & 1.92 \\
    \cline{2-14} \\[-.8em]

    % & \multirow{1}{*}{BERT + BERSON}
    %   & 65.50 & 40.80 & 4.24 & 3.31 & 0.73 & 2.43 & 66.20 & 37.00 & 4.21 & 3.25 & 0.74 & 2.36 \\
    & \multirow{1}{*}{RoBERTa + BERSON}
      & 67.10 & 41.70 & 4.28 & 3.33 & 0.77 & 2.19 & 74.20 & 51.00 & 4.41 & 3.61 & 0.82 & 1.68 \\
    & \multirow{1}{*}{RoBERTa$\dagger$ + BERSON}
      & 72.60 & 49.60 & 4.40 & 3.59 & 0.81 & 1.82 & 76.40 & 56.00 & 4.49 & 3.79 & 0.84 & 1.54 \\
    
    \midrule

    \multirow{8}{*}{Multimodal}
    & \multirow{1}{*}{ViL-BERT + TopoSort}
      & 55.18 & 21.55 & 3.93 & 2.63 & 0.65 & 3.12 & 63.80 & 29.00 & 4.02 & 2.73 & 0.00 & 0.72 \\
    & \multirow{1}{*}{ViL-BERT$\dagger$ + TopoSort}
      & 61.60 & 33.30 & 4.08 & 2.99 & 0.70 & 2.70 & 65.20 & 33.00 & 4.20 & 3.01 & 0.77 & 0.65 \\
    & \multirow{1}{*}{VisualBERT + TopoSort}
      & 63.90 & 33.90 & 4.16 & 3.14 & 0.74 & 2.44 & 65.00 & 33.00 & 4.17 & 3.04 & 0.76 & 2.26 \\
    & \multirow{1}{*}{VisualBERT$\dagger$ + TopoSort}
      & 63.93 & 33.96 & 4.16 & 3.14 & 0.74 & 2.44 & 68.00 & 44.00 & 4.32 & 3.39 & 0.78 & 2.10 \\
    \cline{2-14} \\[-.8em]
    & \multirow{1}{*}{ViL-BERT + BERSON}
      & 69.00 & 45.20 & 4.31 & 3.44 & 0.76 & 2.19 & 74.60 & 53.00 & 4.42 & 3.68 & 0.80 & 1.78 \\
    & \multirow{1}{*}{ViL-BERT$\dagger$ + BERSON}
      & 73.40 & 53.40 & 4.44 & 3.70 & 0.81 & 1.78 & 77.40 & 58.00 & 4.53 & 3.85 & \textbf{0.85} & \textbf{1.44} \\
    & \multirow{1}{*}{VisualBERT + BERSON}
      & 73.80 & 53.60 & 4.44 & 3.70 & 0.81 & 1.78 & 76.20 & 58.00 & 4.49 & 3.85 & 0.83 & 1.58 \\
    & \multirow{1}{*}{VisualBERT$\dagger$ + BERSON}
      & \textbf{75.40} & \textbf{55.50} & \textbf{4.45} & \textbf{3.75} & \textbf{0.82} & \textbf{1.67} & \textbf{78.20} & \textbf{60.00} & \textbf{4.56} & \textbf{3.91} & \textbf{0.85} & \textbf{1.44} \\
    
    \midrule
    
    \multirow{1}{*}{Text-Only}
    & \multirow{1}{*}{\textbf{Human Performance}}
      & \textbf{80.80} & \textbf{63.30} & \textbf{4.58} & \textbf{3.99} & \textbf{0.87} & \textbf{1.25}  & \textbf{82.80} & \textbf{69.00} & \textbf{4.64} & \textbf{4.13} & \textbf{0.88} & \textbf{1.12} \\
    \multirow{1}{*}{Multimodal }
    & \multirow{1}{*}{\textbf{Human Performance}}
      & \textbf{88.20} & \textbf{74.60} & \textbf{4.72} & \textbf{4.32} & \textbf{0.93} & \textbf{0.71}  & \textbf{88.30} & \textbf{77.30} & \textbf{4.76} & \textbf{4.38} & \textbf{0.93} & \textbf{0.73} \\
    
    \bottomrule
    
    \end{tabular}
}
\caption{
\footnotesize
\textbf{Human-Test-Set performance:} $\dagger$ indicates with pretraining. Multimodality is shown consistently helpful, and the BERSON module which exploits global context significantly outperforms the topological sort.
Humans show larger performance gain when images are provided, and are more robust to the local ordering as implied by the smaller gaps between L$_{q}$ and L$_{r}$.
}
\label{tab:model_performances}
% \vspace{-1.5em}
\end{table*}





\iffalse
\begin{table*}[th!]
\centering
\small
\scalebox{.86}{
    \begin{tabular}{cc|cccccc|cccccc}
    \toprule
    \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Modality}}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Models}}} & \multicolumn{6}{c}{\textbf{WikiHow Test Set}} & \multicolumn{6}{c}{\textbf{RecipeQA Test Set}} \\
    % & & & PM$\uparrow$ & EM$\uparrow$ & $\tau\uparrow$ & LC$_{\text{seq}}\uparrow$ & LC$_{\text{str}}\uparrow$ & Dist.$\downarrow$ & PM$\uparrow$ & EM$\uparrow$ & $\tau\uparrow$ & LC$_{\text{seq}}\uparrow$ & LC$_{\text{str}}\uparrow$ & Dist.$\downarrow$ \\
    & & Acc & PMR  & L$_{seq}$ & L$_{str}$ & $\tau$ & Dist. & Acc & PMR & L$_{seq}$ & L$_{str}$ & $\tau$ & Dist. \\
    % & & \textbf{Acc} & \textbf{PMR}  & \textbf{L$_{seq}$} & \textbf{L$_{str}$} & \textbf{$\tau$} & \textbf{Dist.} & \textbf{Acc} & \textbf{PMR}  & \textbf{L$_{seq}$} & \textbf{L$_{str}$} & \textbf{$\tau$} & \textbf{Dist.} \\
    \midrule % \\[-1.1em]
    
    % Test Set.
    
    \multirow{5}{*}{Text-Only}
    & \multirow{1}{*}{RoBERTa + TopoSort}
      & 50.70 & 22.80 & 3.82 & 2.65 & 0.57 & 3.78 & 59.00 & 28.10 & 4.02 & 2.87 & 0.67 & 2.01 \\
    & \multirow{1}{*}{RoBERTa$\dagger$ + TopoSort}
      & 49.30 & 21.40 & 3.79 & 2.61 & 0.55 & 3.94 & 62.80 & 34.10 & 4.14 & 3.07 & 0.72 & 2.56 \\
    \cline{2-14} \\[-.8em]

    & \multirow{1}{*}{BERT + BERSON}
      & 55.90 & 31.90 & 3.98 & 3.03 & 0.60 & 3.51 & 61.20 & 33.20 & 4.10 & 3.04 & 0.68 & 2.82 \\
    & \multirow{1}{*}{RoBERTa + BERSON}
      & 57.40 & 31.20 & 4.01 & 2.98 & 0.64 & 3.21 & 65.80 & 38.86 & 4.20 & 3.24 & 0.74 & 2.37 \\
    & \multirow{1}{*}{RoBERTa$\dagger$ + BERSON}
      & 61.80 & 38.90 & 4.12 & 3.22 & 0.67 & 2.91 & 67.77 & 42.75 & 4.26 & 3.35 & 0.75 & 2.27 \\
    
    \midrule

    \multirow{8}{*}{Multimodal}
    & \multirow{1}{*}{ViL-BERT + TopoSort}
      & 47.29 & 17.04 & 3.69 & 2.43 & 0.53 & 4.08 & 54.50 & 22.70 & 3.90 & 2.63 & 0.64 & 3.21 \\
    & \multirow{1}{*}{ViL-BERT$\dagger$ + TopoSort}
      & 52.90 & 25.30 & 3.88 & 2.73 & 0.60 & 3.57 & 60.30 & 29.50 & 4.04 & 2.88 & 0.69 & 2.81 \\
    & \multirow{1}{*}{VisualBERT + TopoSort}
      & 54.70 & 26.90 & 3.93 & 2.81 & 0.62 & 3.40 & 61.60 & 32.10 & 4.09 & 2.98 & 0.70 & 2.68 \\
    & \multirow{1}{*}{VisualBERT$\dagger$ + TopoSort}
      & 55.20 & 27.80 & 3.94 & 2.84 & 0.62 & 3.38 & 62.50 & 34.60 & 4.14 & 3.11 & 0.70 & 2.69 \\
    \cline{2-14} \\[-.8em]
    & \multirow{1}{*}{ViL-BERT + BERSON}
      & 58.80 & 35.10 & 4.03 & 3.10 & 0.63 & 3.25 & 62.60 & 34.10 & 4.13 & 3.09 & 0.70 & 2.66 \\
    & \multirow{1}{*}{ViL-BERT$\dagger$ + BERSON}
      & 62.70 & 40.10 & 4.16 & 3.28 & 0.68 & 2.83 & 67.33 & 42.62 & 4.28 & 3.41 & 0.75 & 2.28 \\
    & \multirow{1}{*}{VisualBERT + BERSON}
      & 62.00 & 38.50 & 4.12 & 3.23 & 0.67 & 2.89 & 68.42 & 44.43 & \textbf{4.30} & 3.43 & \textbf{0.76} & \textbf{2.18} \\
    & \multirow{1}{*}{VisualBERT$\dagger$ + BERSON}
      & \textbf{63.70} & \textbf{41.00} & \textbf{4.15} & \textbf{3.29} & \textbf{0.69} & \textbf{2.77} & \textbf{68.96} & \textbf{45.34} & \textbf{4.30} & \textbf{3.46} & \textbf{0.76} & 2.19 \\
    
    \bottomrule
    \toprule
    
    % Human Test Set.
    
    \multirow{5}{*}{Text-Only}
    & \multirow{1}{*}{RoBERTa + TopoSort}
      & 60.00 & 30.70 & 4.09 & 2.98 & 0.71 & 2.78 & 69.00 & 41.00 & 4.31 & 3.37 & 0.79 & 2.02 \\
    & \multirow{1}{*}{RoBERTa$\dagger$ + TopoSort}
      & 61.40 & 32.30 & 4.11 & 3.04 & 0.71 & 2.65 & 70.00 & 42.00 & 4.28 & 3.34 & 0.79 & 1.92 \\
    \cline{2-14} \\[-.8em]

    & \multirow{1}{*}{BERT + BERSON}
      & 65.50 & 40.80 & 4.24 & 3.31 & 0.73 & 2.43 & 66.20 & 37.00 & 4.21 & 3.25 & 0.74 & 2.36 \\
    & \multirow{1}{*}{RoBERTa + BERSON}
      & 67.10 & 41.70 & 4.28 & 3.33 & 0.77 & 2.19 & 74.20 & 51.00 & 4.41 & 3.61 & 0.82 & 1.68 \\
    & \multirow{1}{*}{RoBERTa$\dagger$ + BERSON}
      & 72.60 & 49.60 & 4.40 & 3.59 & 0.81 & 1.82 & 76.40 & 56.00 & 4.49 & 3.79 & 0.84 & 1.54 \\
    
    \midrule

    \multirow{8}{*}{Multimodal}
    & \multirow{1}{*}{ViL-BERT + TopoSort}
      & 55.18 & 21.55 & 3.93 & 2.63 & 0.65 & 3.12 & 63.80 & 29.00 & 4.02 & 2.73 & 0.00 & 0.72 \\
    & \multirow{1}{*}{ViL-BERT$\dagger$ + TopoSort}
      & 61.60 & 33.30 & 4.08 & 2.99 & 0.70 & 2.70 & 65.20 & 33.00 & 4.20 & 3.01 & 0.77 & 0.65 \\
    & \multirow{1}{*}{VisualBERT + TopoSort}
      & 63.90 & 33.90 & 4.16 & 3.14 & 0.74 & 2.44 & 65.00 & 33.00 & 4.17 & 3.04 & 0.76 & 2.26 \\
    & \multirow{1}{*}{VisualBERT$\dagger$ + TopoSort}
      & 63.93 & 33.96 & 4.16 & 3.14 & 0.74 & 2.44 & 68.00 & 44.00 & 4.32 & 3.39 & 0.78 & 2.10 \\
    \cline{2-14} \\[-.8em]
    & \multirow{1}{*}{ViL-BERT + BERSON}
      & 69.00 & 45.20 & 4.31 & 3.44 & 0.76 & 2.19 & 74.60 & 53.00 & 4.42 & 3.68 & 0.80 & 1.78 \\
    & \multirow{1}{*}{ViL-BERT$\dagger$ + BERSON}
      & 73.40 & 53.40 & 4.44 & 3.70 & 0.81 & 1.78 & 77.40 & 58.00 & 4.53 & 3.85 & \textbf{0.85} & \textbf{1.44} \\
    & \multirow{1}{*}{VisualBERT + BERSON}
      & 73.80 & 53.60 & 4.44 & 3.70 & 0.81 & 1.78 & 76.20 & 58.00 & 4.49 & 3.85 & 0.83 & 1.58 \\
    & \multirow{1}{*}{VisualBERT$\dagger$ + BERSON}
      & \textbf{75.40} & \textbf{55.50} & \textbf{4.45} & \textbf{3.75} & \textbf{0.82} & \textbf{1.67} & \textbf{78.20} & \textbf{60.00} & \textbf{4.56} & \textbf{3.91} & \textbf{0.85} & \textbf{1.44} \\
    
    \midrule
    
    \multirow{1}{*}{Text-Only}
    & \multirow{1}{*}{\textbf{Human Performance}}
      & \textbf{80.80} & \textbf{63.30} & \textbf{4.58} & \textbf{3.99} & \textbf{0.87} & \textbf{1.25}  & \textbf{82.80} & \textbf{69.00} & \textbf{4.64} & \textbf{4.13} & \textbf{0.88} & \textbf{1.12} \\
    \multirow{1}{*}{Multimodal }
    & \multirow{1}{*}{\textbf{Human Performance}}
      & \textbf{88.20} & \textbf{74.60} & \textbf{4.72} & \textbf{4.32} & \textbf{0.93} & \textbf{0.71}  & \textbf{88.30} & \textbf{77.30} & \textbf{4.76} & \textbf{4.38} & \textbf{0.93} & \textbf{0.73} \\
    
    \bottomrule
    
    \end{tabular}
}
\caption{
\footnotesize
\textbf{Model performance on test set (upper half) and human test set (lower half):} In both sets, multimodal models generally outperform the text-only counterparts. The domain adapting pretraining is shown effective in both language and multimodal models. The BERSON-based ordering module significantly outperforms the topological sort method.
}
\label{tab:model_performances}
\end{table*}
\fi

==> tables/multi_ref_benefits.tex <==
\begin{table}[t!]
\centering
\footnotesize

\scalebox{1.}{
    \begin{tabular}{r|cc}
    \toprule
    \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Dataset}}}
    & \multicolumn{2}{c}{\multirow{1}{*}{\textbf{Benefits from Multi-Reference}}} \\
    & \textbf{Multimodal} & \textbf{Text-Only} \\
    \midrule % \\[-1.1em]
    
    % Human Test Set.
    \multirow{1}{*}{WikiHow}
    & 21.6 \% & 34.7 \%  \\
    \multirow{1}{*}{RecipeQA}
    & 0.0 \%  & 50.0 \%  \\

    \bottomrule
    \end{tabular}
    
}

\caption{
\footnotesize
\textbf{Multi-reference benefits:} We report of what percentage of instances the models benefit from alternative ground truth orders, within each multi-reference subset.
The benefits are defined as if the performance of an instance improves after evaluating with multi-reference ground truths.
}
\label{tab:alternative_benefits}
\end{table}


















\iffalse
\begin{table}[t!]
\centering
\footnotesize

\scalebox{1.}{
    \begin{tabular}{r|ccc}
    \toprule
    \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Dataset}}}
    & \multicolumn{3}{c}{\multirow{1}{*}{\textbf{Multi-reference Beneficial Percentages}}} \\
    & \textbf{Multimodal} & \textbf{Text-Only} & \textbf{Image-Only} \\
    \midrule % \\[-1.1em]
    
    % Human Test Set.
    \multirow{1}{*}{WikiHow}
    & 21.6 \% & 34.7 \%  & 29.2 \%  \\
    \multirow{1}{*}{RecipeQA}
    & 0.0 \%  & 50.0 \%  & 53.9 \%  \\

    \bottomrule
    \end{tabular}
    
}

\caption{
\footnotesize
\textbf{Multi-reference benefits:} We report of what percentage of instances the models benefit from alternative ground truth orders, within each multi-reference subset.
The benefits are defined as if the performance of an instance improves after evaluating with multi-reference ground truths.
}
\label{tab:alternative_benefits}
\end{table}
\fi

==> tables/multi_ref_performance.tex <==
\begin{table*}[th!]
\centering
\small
\scalebox{.87}{
    \begin{tabular}{cccc|cccccc|cccccc}
    \toprule
    \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Modality}}}
    & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Subset}}}
    & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Eval.}}}
    & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Type}}} 
    & \multicolumn{6}{c}{\textbf{WikiHow Golden-Test-Set}}
    % & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Subset}}}
    & \multicolumn{6}{c}{\textbf{RecipeQA Golden-Test-Set}} \\
    & & &
    & Acc$\uparrow$ & PMR$\uparrow$ & L$_{q}\uparrow$ & L$_{r}\uparrow$ & $\tau\uparrow$ & Dist$\downarrow$
    & Acc$\uparrow$ & PMR$\uparrow$ & L$_{q}\uparrow$ & L$_{r}\uparrow$ & $\tau\uparrow$ & Dist$\downarrow$ \\
    \midrule
    
    \multirow{10}{*}{Image-Only}
    & \multirow{1}{*}{Single} & Single & Perf.
      & 28.38 & 5.05 & 3.09 & 1.97 & 0.15 & 6.84 & 49.89 & 17.24 & 3.75 & 2.47 & 0.55 & 3.84 \\
    & \multirow{1}{*}{Multi.} & Single & Perf.
      & 26.67 & 4.17 & 3.08 & 1.83 & 0.24 & 6.42 & 29.23 & 7.69 & 3.23 & 1.92 & 0.28 & 6.00 \\
    & \multirow{1}{*}{Multi.} & Multi.& Perf.
      & 39.17 & 8.33 & 3.21 & 1.92 & 0.29 & 5.58 & 40.00 & 7.69 & 3.38 & 2.31 & 0.29 & 5.69 \\
    & \multirow{1}{*}{All} & Multi. & Perf.
      & 29.24 & 5.32 & 3.10 & 1.97 & 0.16 & 6.74 & 48.60 & 16.00 & 3.70 & 2.45 & 0.52 & 4.08 \\
    & \multirow{1}{*}{---} & --- & Gain
      & 3.54 & 6.83 & 0.32 & 0.51 & 0.0 & 0.88 & 2.97 & 0.00 & 0.54 & 2.08 & 0.39 & 0.97 \\
    \cline{2-16} \\[-.8em]
    & \multirow{1}{*}{Single} & Single & $\dagger$Perf.
      & 68.47 & 48.36 & 4.29 & 3.54 & 0.73 & 2.38 & 81.61 & 66.67 & 4.58 & 4.10 & 0.87 & 1.21 \\
    & \multirow{1}{*}{Multi.} & Single & $\dagger$Perf.
      & 64.58 & 37.50 & 4.02 & 3.19 & 0.63 & 2.96 & 72.31 & 50.00 & 4.31 & 3.50 & 0.80 & 1.85 \\
    & \multirow{1}{*}{Multi.} & Multi.& $\dagger$Perf.
      & 75.83 & 56.25 & 4.23 & 3.71 & 0.70 & 2.38 & 79.23 & 61.54 & 4.50 & 3.88 & 0.82 & 1.54 \\
    & \multirow{1}{*}{All} & Multi. & $\dagger$Perf.
      & 69.06 & 48.99 & 4.28 & 3.55 & 0.73 & 2.38 & 81.30 & 66.00 & 4.57 & 4.07 & 0.87 & 1.25 \\
    & \multirow{1}{*}{---} & --- & $\dagger$Gain
      & 1.32 & 3.16 & 0.39 & 1.19 & 0.69 & 1.92 & 1.12 & 2.33 & 0.55 & 1.24 & 0.35 & 3.10 \\
      
    \midrule
      
    \multirow{10}{*}{Text-Only}
    & \multirow{1}{*}{Single} & Single & Perf.
      & 77.30 & 62.30 & 4.54 & 3.98 & 0.83 & 1.59 & 79.32 & 60.23 & 4.53 & 3.90 & 0.86 & 1.30 \\
    & \multirow{1}{*}{Multi.} & Single & Perf.
      & 67.35 & 40.82 & 4.31 & 3.35 & 0.76 & 2.20 & 60.00 & 33.33 & 4.17 & 3.17 & 0.68 & 2.83 \\
    & \multirow{1}{*}{Multi.} & Multi.& Perf.
      & 80.00 & 59.18 & 4.47 & 3.86 & 0.87 & 1.43 & 75.00 & 58.33 & 4.50 & 3.92 & 0.80 & 1.83 \\
    & \multirow{1}{*}{All} & Multi. & Perf.
      & 77.74 & 61.79 & 4.53 & 3.96 & 0.83 & 1.56 & 78.80 & 60.00 & 4.53 & 3.90 & 0.86 & 1.36 \\
    & \multirow{1}{*}{---} & --- & Gain
      & 2.72 & 5.09 & 0.67 & 2.33 & 1.22 & 7.69 & 2.34 & 5.26 & 0.89 & 2.36 & 1.66 & 8.11 \\
    \cline{2-16} \\[-.8em]
    & \multirow{1}{*}{Single} & Single & $\dagger$Perf.
      & 85.57 & 71.41 & 4.68 & 4.24 & 0.90 & 0.92 & 90.27 & 80.41 & 4.80 & 4.47 & 0.94 & 0.59 \\
    & \multirow{1}{*}{Multi.} & Single & $\dagger$Perf.
      & 72.03 & 43.84 & 4.36 & 3.46 & 0.81 & 1.75 & 79.00 & 65.00 & 4.45 & 3.95 & 0.82 & 1.50 \\
    & \multirow{1}{*}{Multi.} & Multi.& $\dagger$Perf.
      & 85.51 & 71.38 & 4.62 & 4.14 & 0.87 & 1.04 & 87.00 & 80.00 & 4.70 & 4.40 & 0.88 & 1.10 \\
    & \multirow{1}{*}{All} & Multi. & $\dagger$Perf.
      & 85.56 & 71.40 & 4.67 & 4.22 & 0.90 & 0.94 & 89.88 & 80.36 & 4.79 & 4.46 & 0.93 & 0.66 \\
    & \multirow{1}{*}{---} & --- & $\dagger$Gain
      & 2.64 & 6.72 & 0.91 & 2.71 & 1.15 & 10.88 & 1.08 & 2.29 & 0.63 & 1.22 & 0.78 & 6.83 \\
      
    \midrule
      
    \multirow{10}{*}{Multimodal}
    & \multirow{1}{*}{Single} & Single & Perf.
      & 81.68 & 69.60 & 4.62 & 4.15 & 0.86 & 1.31 & 83.71 & 69.07 & 4.62 & 4.12 & 0.89 & 1.01 \\
    & \multirow{1}{*}{Multi.} & Single & Perf.
      & 70.98 & 47.06 & 4.35 & 3.59 & 0.78 & 2.08 & 46.67 & 33.33 & 4.33 & 3.67 & 0.60 & 4.00 \\
    & \multirow{1}{*}{Multi.} & Multi.& Perf.
      & 78.82 & 60.78 & 4.49 & 3.90 & 0.81 & 1.61 & 60.00 & 33.33 & 4.33 & 3.78 & 0.73 & 2.67 \\
    & \multirow{1}{*}{All} & Multi. & Perf.
      & 81.19 & 68.10 & 4.60 & 4.11 & 0.85 & 1.36 & 83.00 & 68.00 & 4.61 & 4.11 & 0.89 & 1.06 \\
    & \multirow{1}{*}{---} & --- & Gain
      & 1.67 & 3.55 & 0.51 & 1.32 & 0.71 & 5.55 & 0.48 & 0.00 & 0.00 & 0.08 & 0.44 & 3.63 \\
    \cline{2-16} \\[-.8em]
    & \multirow{1}{*}{Single} & Single & $\dagger$Perf.
      & 92.86 & 83.67 & 4.82 & 4.56 & 0.96 & 0.41 & 91.88 & 82.61 & 4.81 & 4.52 & 0.95 & 0.46 \\
    & \multirow{1}{*}{Multi.} & Single & $\dagger$Perf.
      & 82.09 & 59.80 & 4.56 & 3.99 & 0.89 & 1.05 & 100.00 & 100.00 & 5.00 & 5.00 & 1.00 & 0.00 \\
    & \multirow{1}{*}{Multi.} & Multi.& $\dagger$Perf.
      & 92.22 & 83.33 & 4.79 & 4.54 & 0.94 & 0.54 & 100.00 & 100.00 & 5.00 & 5.00 & 1.00 & 0.00 \\
    & \multirow{1}{*}{All} & Multi. & $\dagger$Perf.
      & 92.75 & 83.61 & 4.82 & 4.55 & 0.95 & 0.44 & 92.12 & 83.13 & 4.82 & 4.53 & 0.95 & 0.45 \\
    & \multirow{1}{*}{---} & --- & $\dagger$Gain
      & 1.89 & 5.02 & 0.84 & 2.08 & 0.87 & 16.41 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\

    \bottomrule
    
    \end{tabular}
}
\caption{
\footnotesize
\textbf{Multi-reference performance with alternative orders:} $\dagger$ denotes results from human performance. We include performance of each subset categorized by whether the instance have more than one ground truth orders (denoted as \textbf{Multi.}) or just the original ground truth order (denoted as \textbf{Single}). For the multi-reference subset, we show the performance evaluated (\textbf{Eval}) using either single or multiple reference. Performance are denoted as \textbf{Perf.} type where as \textbf{Gain} denotes the performance gain (in percentage) of the overall multi-reference performance compared to the performance in~\tbref{tab:model_performances}.
}
\label{tab:multiref_perf}
% \vspace{-1.5em}
\end{table*}












\iffalse
\begin{table}[th!]
\centering
\small
\scalebox{0.79}{
    \begin{tabular}{cc|cccccc}
    \toprule
    \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Modality}}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Type}}} &
    \multicolumn{6}{c}{\textbf{WikiHow Golden-Test-Set}} \\
    & & Acc$\uparrow$ & PMR$\uparrow$  & L$_{q}\uparrow$ & L$_{r}\uparrow$ & $\tau\uparrow$ & Dist$\downarrow$ \\
    \midrule % \\[-1.1em]
    
    % Human Test Set.
    
    \multirow{4}{*}{Image-Only}
    & \multirow{1}{*}{Perf.}
      & 00.00 & 00.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
    & \multirow{1}{*}{Gain}
      & 00.00 & 00.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
    \cline{2-8} \\[-.8em]
    & \multirow{1}{*}{$\dagger$Perf.}
      & 69.17 & 49.17 & 4.29 & 3.56 & 0.73 & 2.37 \\
    & \multirow{1}{*}{$\dagger$Gain}
      & 8.08  & 14.35 & 2.63 & 5.95 & 7.35 & 14.13 \\
    \midrule
    
    \multirow{4}{*}{Text-Only}
    & \multirow{1}{*}{Perf.}
      & 00.00 & 00.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
    & \multirow{1}{*}{Gain}
      & 00.00 & 00.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
    \cline{2-8} \\[-.8em]
    & \multirow{1}{*}{$\dagger$Perf.}
      & 85.78 & 71.99 & 4.68 & 4.24 & 0.90 & 0.92 \\
    & \multirow{1}{*}{$\dagger$Gain}
      & 3.35  & 6.97  & 1.08 & 2.91 & 1.12 & 11.54 \\
    \midrule
    
    \multirow{4}{*}{Multimodal}
    & \multirow{1}{*}{Perf.}
      & 00.00 & 00.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
    & \multirow{1}{*}{Gain}
      & 00.00 & 00.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
    \cline{2-8} \\[-.8em]
    & \multirow{1}{*}{$\dagger$Perf.}
      & 92.15 & 82.42 & 4.81 & 4.52 & 0.95 & 0.47 \\
    & \multirow{1}{*}{$\dagger$Gain}
      & 2.39  & 6.62  & 1.05 & 2.73 & 1.06 & 18.97 \\
    
    \bottomrule
    
    \toprule
    \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Modality}}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Refs.}}} &
    \multicolumn{6}{c}{\textbf{RecipeQA Golden-Test-Set}} \\
    & & Acc$\uparrow$ & PMR$\uparrow$  & L$_{q}\uparrow$ & L$_{r}\uparrow$ & $\tau\uparrow$ & Dist$\downarrow$ \\
    \midrule % \\[-1.1em]
    
    \multirow{4}{*}{Image-Only}
    & \multirow{1}{*}{Perf.}
      & 00.00 & 00.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
    & \multirow{1}{*}{Gain}
      & 00.00 & 00.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
    \cline{2-8} \\[-.8em]
    & \multirow{1}{*}{$\dagger$Perf.}
      & 81.30 & 66.00 & 4.57 & 4.07 & 0.87 & 1.25 \\
    & \multirow{1}{*}{$\dagger$Gain}
      & 1.62  & 1.54  & 0.44 & 1.24 & 1.16 & 3.10 \\
    \midrule
    
    \multirow{4}{*}{Text-Only}
    & \multirow{1}{*}{Perf.}
      & 00.00 & 00.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
    & \multirow{1}{*}{Gain}
      & 00.00 & 00.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
    \cline{2-8} \\[-.8em]
    & \multirow{1}{*}{$\dagger$Perf.}
      & 89.29 & 79.35 & 4.77 & 4.43 & 0.93 & 0.70 \\
    & \multirow{1}{*}{$\dagger$Gain}
      & 0.33  & 1.73  & 0.42 & 0.68 & 1.09 & 5.41 \\
    \midrule
    
    \multirow{4}{*}{Multimodal}
    & \multirow{1}{*}{Perf.}
      & 00.00 & 00.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
    & \multirow{1}{*}{Gain}
      & 00.00 & 00.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
    \cline{2-8} \\[-.8em]
    & \multirow{1}{*}{$\dagger$Perf.}
      & 92.12 & 83.12 & 4.82 & 4.53 & 0.95 & 0.45 \\
    & \multirow{1}{*}{$\dagger$Gain}
      & 0.13  & 0.14 & 0.21  & 0.44 & 0.00 & 6.25 \\
    \bottomrule
    
    \end{tabular}
}
\caption{
\footnotesize
\textbf{Multi-Ref:} ... $\dagger$ denotes humna performance...
}
\label{tab:multiref_gain}
% \vspace{-1.5em}
\end{table}
\fi

==> tables/single_model_performance.tex <==
\begin{table*}[th!]
\centering
\small
\scalebox{0.8}{
    \begin{tabular}{crr|cccccc}
    \toprule
    \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Modality}}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Models}}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Pretraining}}} &
    \multicolumn{6}{c}{\textbf{WikiHow Golden-Test-Set}} \\
    & & & Acc$\uparrow$ & PMR$\uparrow$  & L$_{q}\uparrow$ & L$_{r}\uparrow$ & $\tau\uparrow$ & Dist$\downarrow$ \\
    \midrule
    
    \multirow{6}{*}{Image-Only}
    & \multirow{1}{*}{ResNet} & \multirow{1}{*}{---}
      & 00.00 & 00.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
    & \multirow{1}{*}{ResNet} & \multirow{1}{*}{ImgSwap}
      & 00.00 & 00.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
    \cline{2-9} \\[-.8em]
    & \multirow{1}{*}{CLIP} & \multirow{1}{*}{---}
      & 00.00 & 00.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
    & \multirow{1}{*}{CLIP} & \multirow{1}{*}{ImgSwap}
      & 00.00 & 00.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
    & \multirow{1}{*}{CLIP} & \multirow{1}{*}{ImgSwap + P-ImgSwap}
      & 00.00 & 00.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
    & \multirow{1}{*}{CLIP} & \multirow{1}{*}{MRM + ImgSwap + P-ImgSwap}
      & 23.12 & 4.98 & 2.97 & 1.92 & 0.08 & 7.50 \\
    \midrule
    
    \multirow{2}{*}{Text-Only}
    & \multirow{1}{*}{RoBERTa} & \multirow{1}{*}{---}
      & 00.00 & 00.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
    & \multirow{1}{*}{RoBERTa} & \multirow{1}{*}{MLM}
      & 00.00 & 00.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
    \midrule

    \multirow{9}{*}{Multimodal}
    & \multirow{1}{*}{VisualBERT} & \multirow{1}{*}{---}
      & 75.30 & 57.10 & 4.45 & 3.83 & 0.81 & 1.65 \\
    & \multirow{1}{*}{VisualBERT} & \multirow{1}{*}{MLM + ImgSwap}
      & 77.30 & 59.40 & 4.50 & 3.86 & 0.83 & 1.58 \\
    \cline{2-9} \\[-.8em]
    
    & \multirow{1}{*}{VisualBERT-CLIP} & \multirow{1}{*}{---}
      & 76.15 & 58.80 & 4.49 & 3.87 & 0.82 & 1.68 \\
    & \multirow{1}{*}{VisualBERT-CLIP} & \multirow{1}{*}{MLM}
      & 77.87 & 60.47 & 4.54 & 3.94 & 0.85 & 1.48 \\
    & \multirow{1}{*}{VisualBERT-CLIP} & \multirow{1}{*}{MLM + ImgSwap}
      & 78.21 & 62.13 & 4.55 & 3.97 & 0.84 & 1.50 \\
    & \multirow{1}{*}{VisualBERT-CLIP} & \multirow{1}{*}{MLM + ImgSwap + P-ImgSwap}
      & 79.00 & 64.12 & 4.58 & 4.04 & 0.85 & 1.47 \\
    & \multirow{1}{*}{VisualBERT-CLIP} & \multirow{1}{*}{MLM + M(ImgSwap + P-ImgSwap)}
      & 00.00 & 00.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
    & \multirow{1}{*}{VisualBERT-CLIP} & \multirow{1}{*}{MLM + MRM}
      & 00.00 & 00.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
    \midrule

    \multirow{1}{*}{Image-Only}
    & \multirow{1}{*}{\textbf{Human Performance}}
      & --- & \textbf{64.00} & \textbf{43.00} & \textbf{4.18} & \textbf{3.36} & \textbf{0.68} & \textbf{2.76} \\
    \multirow{1}{*}{Text-Only}
    & \multirow{1}{*}{\textbf{Human Performance}}
      & --- & \textbf{83.00} & \textbf{67.30} & \textbf{4.63} & \textbf{4.12} & \textbf{0.89} & \textbf{1.04} \\
    \multirow{1}{*}{Multimodal}
    & \multirow{1}{*}{\textbf{Human Performance}}
      & --- & \textbf{90.00} & \textbf{77.30} & \textbf{4.76} & \textbf{4.40} & \textbf{0.94} & \textbf{0.58} \\
    \bottomrule
    
    \toprule
    \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Modality}}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Models}}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Pretraining}}} &
    \multicolumn{6}{c}{\textbf{RecipeQA Golden-Test-Set}} \\
    & & & Acc$\uparrow$ & PMR$\uparrow$  & L$_{q}\uparrow$ & L$_{r}\uparrow$ & $\tau\uparrow$ & Dist$\downarrow$ \\
    \midrule
    
    \multirow{6}{*}{Image-Only}
    & \multirow{1}{*}{ResNet} & \multirow{1}{*}{---}
      & 00.00 & 00.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
    & \multirow{1}{*}{ResNet} & \multirow{1}{*}{ImgSwap}
      & 00.00 & 00.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
    \cline{2-9} \\[-.8em]
    & \multirow{1}{*}{CLIP} & \multirow{1}{*}{---}
      & 00.00 & 00.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
    & \multirow{1}{*}{CLIP} & \multirow{1}{*}{ImgSwap}
      & 00.00 & 00.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
    & \multirow{1}{*}{CLIP} & \multirow{1}{*}{ImgSwap + P-ImgSwap}
      & 00.00 & 00.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
    & \multirow{1}{*}{CLIP} & \multirow{1}{*}{MRM + ImgSwap + P-ImgSwap}
      & 00.00 & 00.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
    \midrule
    
    \multirow{2}{*}{Text-Only}
    & \multirow{1}{*}{RoBERTa} & \multirow{1}{*}{---}
      & 00.00 & 00.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
    & \multirow{1}{*}{RoBERTa} & \multirow{1}{*}{MLM}
      & 00.00 & 00.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
    \midrule

    \multirow{9}{*}{Multimodal}
    & \multirow{1}{*}{VisualBERT} & \multirow{1}{*}{---}
      & 00.00 & 00.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
    & \multirow{1}{*}{VisualBERT} & \multirow{1}{*}{MLM + ImgSwap}
      & 00.00 & 00.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
    \cline{2-9} \\[-.8em]
    & \multirow{1}{*}{VisualBERT-CLIP} & \multirow{1}{*}{---}
      & 76.15 & 58.80 & 4.49 & 3.87 & 0.82 & 1.68 \\
    & \multirow{1}{*}{VisualBERT-CLIP} & \multirow{1}{*}{MLM}
      & 77.87 & 60.47 & 4.54 & 3.94 & 0.85 & 1.48 \\
    & \multirow{1}{*}{VisualBERT-CLIP} & \multirow{1}{*}{MLM + ImgSwap}
      & 00.00 & 00.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
    & \multirow{1}{*}{VisualBERT-CLIP} & \multirow{1}{*}{MLM + ImgSwap + P-ImgSwap}
      & 00.00 & 00.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
    & \multirow{1}{*}{VisualBERT-CLIP} & \multirow{1}{*}{MLM + M(ImgSwap + P-ImgSwap)}
      & 00.00 & 00.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
    & \multirow{1}{*}{VisualBERT-CLIP} & \multirow{1}{*}{MLM + MRM}
      & 00.00 & 00.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
    \midrule

    \multirow{1}{*}{Image-Only}
    & \multirow{1}{*}{\textbf{Human Performance}}
      & --- & \textbf{80.00} & \textbf{65.00} & \textbf{4.55} & \textbf{4.02} & \textbf{0.86} & \textbf{1.29} \\
    \multirow{1}{*}{Text-Only}
    & \multirow{1}{*}{\textbf{Human Performance}}
      & --- & \textbf{89.00} & \textbf{78.00} & \textbf{4.75} & \textbf{4.40} & \textbf{0.92} & \textbf{0.74} \\
    \multirow{1}{*}{Multimodal}
    & \multirow{1}{*}{\textbf{Human Performance}}
      & --- & \textbf{92.00} & \textbf{83.00} & \textbf{4.81} & \textbf{4.51} & \textbf{0.95} & \textbf{0.48} \\
    \bottomrule
    
    \end{tabular}
}
\caption{
\footnotesize
\telin{Change this table to two column dataset side by side, shorten the names and prepare this for ablation table}
\textbf{NEW SINGLE Human-Test-Set performance:} $\dagger$ indicates with pretraining. Multimodality is shown consistently helpful, and the BERSON module which exploits global context significantly outperforms the topological sort.
Humans show larger performance gain when images are provided, and are more robust to the local ordering as implied by the smaller gaps between L$_{q}$ and L$_{r}$.
}
\label{tab:model_performances}
% \vspace{-1.5em}
\end{table*}

==> tables/zero_shot_ret.tex <==
\begin{table}[t!]
\centering
\small
\setlength{\tabcolsep}{3pt}
\scalebox{.87}{
    \begin{tabular}{r|ccc|ccc}
    \toprule
    \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Model}}} & \multicolumn{3}{c}{\textbf{WikiHow}} & \multicolumn{3}{c}{\textbf{RecipeQA}} \\
    & MRR$\uparrow$ & Top-1$\uparrow$  & MRSR$\uparrow$ & MRR$\uparrow$ & Top-1$\uparrow$ & MRSR$\uparrow$ \\
    \midrule % \\[-1.1em]
    
    % Human Test Set.
    \multirow{1}{*}{Text-Only}
    & 0.341          &  14.9          & 0.195          & 0.265           & 8.0           & 0.163 \\
    \multirow{1}{*}{Multimodal}
    & \textbf{0.347} & \textbf{16.8}  & \textbf{0.230} & \textbf{0.428}  & \textbf{25.0} & \textbf{0.275} \\
    
    \bottomrule
    
    \end{tabular}
}
\caption{
\footnotesize
\textbf{Zero-shot manual completion:}
    % The model is asked to retrieve a missing step from an \textit{incomplete} instructional manual and correctly put the retrieved step back to its proper position.
    The results are obtained from the best performing multimodal (VisualBERT$\dagger$ + BERSON) and text-only (RoBERTa$\dagger$ + BERSON) models.
}
\label{tab:zero_shot}
\vspace{-1.5em}
\end{table}
